Losing Treewidth by Separating Subsets

We study the problem of deleting the smallest set $S$ of vertices (resp. edges) from a given graph $G$ such that the induced subgraph (resp. subgraph) $G \setminus S$ belongs to some class $\mathcal{H}$. We consider the case where graphs in $\mathcal{H}$ have treewidth bounded by $t$, and give a general framework to obtain approximation algorithms for both vertex and edge-deletion settings from approximation algorithms for certain natural graph partitioning problems called $k$-Subset Vertex Separator and $k$-Subset Edge Separator, respectively. For the vertex deletion setting, our framework combined with the current best result for $k$-Subset Vertex Separator, yields a significant improvement in the approximation ratios for basic problems such as $k$-Treewidth Vertex Deletion and Planar-$F$ Vertex Deletion. Our algorithms are simpler than previous works and give the first uniform approximation algorithms under the natural parameterization. For the edge deletion setting, we give improved approximation algorithms for $k$-Subset Edge Separator combining ideas from LP relaxations and important separators. We present their applications in bounded-degree graphs, and also give an APX-hardness result for the edge deletion problems.

==> lowerbounds.tex <==
\begin{lemma}
If \VP admits an $(\alpha_k,\, \Oh(1))$-bicriteria approximation, then Theorem~\ref{lem:main} can be improved to guarantee $\Oh(1)$-approximation in FPT time.
\end{lemma}
\begin{proof}
The reasoning is the same as before.
We choose $\beta_k = \Oh(1)$ that ensures decrease of the solution candidate two times per iteration.
The resulting running time is $\Oh^*(f(t\cdot\alpha_t)) + n^{\Oh(1)}$.
\end{proof}

\begin{lemma}\label{lem:treewidth2pt-hardness}
If \textsc{Treewidth $t$-Deletion} admits an $\Oh(1)$-approximation in FPT time,
then the same applies to \PT.
\end{lemma}\begin{proof}
Since $k$-path-free graphs have treewidth bounded by $k$~\cite{treedepth},
there is a set $S \subseteq V(G),\, |S| \le \OPT$ such that $tw(G \sm S) \le k$.
We launch the algorithm for \textsc{Treewidth $t$-Deletion} to find
a set $S' \subseteq V(G)$ being an $\Oh(1)$-approximation
and construct the corresponding tree decomposition.

Assume now that we have a solution candidate $R$.
We can use Lemma~\ref{lem:cut} with $\delta = 4k$ to obtain a set $Y \subseteq V(G),\, |Y| \le \frac{|R|}{4}$ such that each connected component $C \subseteq G \sm Y$ has at most $4k$ vertices from $R$.
We solve \PT exactly on each $C$ (see Lemma~\ref{lem:pt}) and denote the union of solutions, plus $S' \cup Y$, as $R'$.
Assuming $R$ is an $\alpha$-approximate solution,
we have $|R'| \le \big(\Oh(1) + \frac{\alpha}{4}\big)\cdot \OPT$.
As long as $\alpha$ is 4 times larger than the first summand, we deduce that $|R'| \le \frac{|R|}{2}$.
After repeating the procedure $\Oh(\log n)$ times, we get an $\Oh(1)$-approximation.
\end{proof}

\begin{corollary}
The presented reductions preserve running times of type $f(k)n^{g(k)}$ as well.
\end{corollary}

\begin{theorem}
Under UGC, there can be no $(\alpha_k,\, 2-\eps)$-bicriteria approximation for \VP.
\end{theorem}
\begin{proof}
We are going to approximate \textsc{Feedback Vertex Set}, which is known to be UGC-hard to approximate under factor 2.
For the sake of simplicity, the approximation ratio obtained in Theorem~\ref{lem:main} and Lemma~\ref{lem:treewidth2pt-hardness}
is 4 times larger than the ratio for \VP.
However, we can replace 4 with $(1+\frac{\eps}{2})$ by increasing the constant in $\beta_k$
and the number of iterations of the algorithm.
The obtained approximation factor is less than 2 and the bound $\delta$ on the solution size in each connected component is constant, so the running time remains polynomial.
\end{proof}

\begin{problem}
Can we establish a superconstant hardness of approximation for \PT (or any other family of planar graphs) under UGC?
\end{problem}
